Distance dependence of angular correlations in dense polymer solutions

Angular correlations in dense solutions and melts of flexible polymer chains are investigated with respect to the distance $r$ between the bonds by comparing quantitative predictions of perturbation calculations with numerical data obtained by Monte Carlo simulation of the bond-fluctuation model. We consider both monodisperse systems and grand-canonical (Flory-distributed) equilibrium polymers. Density effects are discussed as well as finite chain length corrections. The intrachain bond-bond correlation function $P(r)$ is shown to decay as $P(r) \sim 1/r^3$ for $\xi \ll r \ll \r^*$ with $\xi$ being the screening length of the density fluctuations and $r^* \sim N^{1/3}$ a novel length scale increasing slowly with (mean) chain length $N$.

==> answer <==
Ref.: ma-2009-02299h

Dear Prof. Lipson,

thank you very much for your message containing the referee reports
concerning our manuscript

  Distance dependence of angular correlations in dense polymer solutions 
  Wittmer, Johner, Obukhov, Meyer, Cavallo, Baschnagel.

We are pleased to hear that both referees appreciate our work and that
they only have a few minor remarks. As shown below all the points raised 
can be readily addressed. We are particulary grateful to the second referee 
for his or her detailed and thoughtful comments. 

We hope that in its present form the paper is now ready for publication.

Sincerly yours, Joachim Wittmer


First referee:
=============

> 1) pg 1 line 45: move the reference “10” some where else on the line 
> (away from the power “2” in the equation).

We have changed this.

> 2) pg 3 line 4: check should this be eq. 4 or eq 5?

The referee is right. It is eq 5. We have changed this.

> 3) pg 9 line 42: should be “corresponds”

We have changed this.


Second referee:
===============

> 1) Page 1, line 41: most probably the authors meant to write b2 = R2 / N 
> as they use the same expression for b as for chain stiffness. 

To clarify this we have changed in line 40

  "R(N) the typical chain size" --> "R(N) the root-mean-square end-to-end distance"

and have given the definition of $b$ in the next line 
  
  "b \equiv \lim_{N\to \infty} R(N)/N^{1/2}" 

following Edwards [2]. We want to introduce here the stiffness parameter $c_{\infty} = (b/l)^2$,
the only relevant parameter of the theory.
 
> 2) Page 1, line 53: in addition to references 11-13 very recently an independent simulation 
> study based on off-lattice MC simulations (Phys. Rev. Lett. 2008, 100, 050602) also showed 
> deviation from Flory´s ideality hypothesis. 

Please note that we address in this paper 

- universal physics relevant for asymptotically large chains 
- on large length scales, much larger than any monomeric length
- for systems in thermal equilibrium 
- for polymer solutions without any (local or global) crystallization effects.

Deviations to Flory's ideality hypothesis are of course expected where one or several of the 
above conditions are not satisfied. The paper mentioned by the referee is, hence, only of
marginal relevence to the presented work.

Please note also that local and non-universal physics, such as packing effects, must indeed
influence properties such as $b$, $l$, $c_{\infty}$ or $\xi$ and, possibly, their density 
dependence at high volume fractions. As long as the chains remain (essentially) Gaussian on 
large scales these are, however, prefactor effects which are taken into account by using the 
_measured_ parameter $c_{\infty}(\rho)$ for each density.

> 3) Page 3, line 56: the authors could add "in Fig. 1b" after "bold arrows". 

We have changed this.

> 4) In the titles of the paragraphs extracting the bond-bond correlation functions 
> in pages 5-7 the authors could add "fully flexible" as in all studied cases coo=1. 

We have clearly stated at the end of the first paragraph of section II on page 3 
that we first focus on flexible chains. To stress this fact we have changed the 
paragraph title "Reciprocal space" on page 3 to "Reciprocal space description of
flexible chains". We see no need to repeat this in the titles of the following paragraphs. 

> 5) Page 6, line 22: the authors should add that self-assembly does not include the 
> formation of branches along the chain backbones (linear chains).

We have changed "(no closed loops being allowed)" to
"(branching of chains and formation of closed loops being disallowed)".

> 6) The authors employ chain-connectivity-altering MC moves (double bridging) for the 
> equilibration of monodisprse linear chains. Double bridging and related moves can be 
> modified, through the employment of appropriate chemical potentials, to be applicable 
> to Flory-distributed chains. Obviously afforded MC-based equilibration in such systems 
> is much faster than in strictly monodisperse ones. Did the authors use such an approach? 

The monodisperse chains presented (Fig. 2 and 3) are strictly monodisperse and the 
chain-connectivity-altering Monte Carlo moves obey this contraint rigorously at each step. 
As the referee correctly states this (and other reasons related to the strong return 
probability to an original topological state) makes the double-bridging algorithm much 
less attractive for large $N \gg 1000$ as was originally hoped for by Theodorou and others. 
The equilibration of the chain length $N=8192$ was, hence, a computational challenge 
which took us several years. How this is done and tested is explained in detail in Ref.[7].
This paper also contains some information on the dynamical behavior of the algorithm. 

We do not exclude that other algorithms (using, e.g., grand-canonical moves) might turn out 
to be more effective for monodisperse chains. The important point is here that we use a well 
tested and documented configuration ensemble for rigorously monodisperse chains.

> From the related discussion in section 3 (page 9) it is not clear to me whether the same 
> MC scheme was used in both simulated systems (monodisperse and Flory) or not.

As the referee states it helps a lot if one does not insist on the monodispersity contraint
and especially the simulation of equilibrium polymers which are allowed to break reversibly
everywhere along the chain contour turns out to be very efficient. For this reason it was
only necessary to use local Monte Carlo moves. This is clearly stated at the end of section III.

Please note that we only use canonical Monte Carlo moves, i.e. that neither volume nor
particle number is allowed to fluctuate. Since the algorithm is rather standard and has 
been described in all detail in Refs. [15,28] we do not see the need to give additional 
information in the paper.

> 7)Very recent studies (Phys. Rev. Lett. 2009, 101, 265702) suggest that at very high densities 
> the semi-dilute regime is succeeded by the marginal one where chains collapse in size as quantified 
> by a scalign exponent of -1. I wonder if the authors have simulated systems at high enough densities 
> so that the density dependence on chain stiffness should change from -0.23 to -1 as the authors 
> suggest that eqs 37 and 38 are adequate for the whole density range.

As already explained with respect to point (2) the chain stiffness, the effective bond length $b$ 
or the screening length $\xi$ of the solution may do what they want as a function of density 
(or other parameters). In fact the power-law scaling for $b$ and $\xi$ (eqs 37 and 38) is indeed 
not rigorous (inset of fig 2(b)), as we have clearly stated in the draft. But in turns of the 
_measured_ values of $b$ and $\xi$ this is irrelevant for the data collapse (main figure 2(b)) 
we want to demonstrate.

We have been puzzled where to quote the (in general) interesting papers suggested by the 
referee and have finally decided to mention 

    PRL 101, 256702 (2008)

due to the somewhat related figure 1 at the bottom of page 10 where we hint 
to the breakdown of the semi-dilute regime.

As a matter of fact using a BFM version with finite overlap penalty (described in Ref. [9]) 
we have simulated much larger volume fractions without observing any qualitative different 
behavior for the scaling of the bond-bond correlation function $P(r)$. 

> 8)Page 11, figure legend: "The data approach" instead of "The data approaches".

Has been changed. 



